SCALOFT: An Initial Approach for Situation Coverage-Based Safety Analysis of an Autonomous Aerial Drone in a Mine Environment

The safety of autonomous systems in dynamic and hazardous environments poses significant challenges. This paper presents a testing approach named SCALOFT for systematically assessing the safety of an autonomous aerial drone in a mine. SCALOFT provides a framework for developing diverse test cases, real-time monitoring of system behaviour, and detection of safety violations. Detected violations are then logged with unique identifiers for detailed analysis and future improvement. SCALOFT helps build a safety argument by monitoring situation coverage and calculating a final coverage measure. We have evaluated the performance of this approach by deliberately introducing seeded faults into the system and assessing whether SCALOFT is able to detect those faults. For a small set of plausible faults, we show that SCALOFT is successful in this.

==> Extrawriting.tex <==
 Here, we will detail the mathematical logic underlying this approach. 

The initial coverage grid is defined  as a combination of predefined waypoints and the elements from the target situation space (See Table 2).

Let \( W_1, W_2, \dots, W_n \) represent the waypoints in the mine, where each waypoint \( W_i \) is a three-dimensional vector:
\[
W_i = (X_i, Y_i, Z_i), \quad i = 1, 2, \dots, n
\]
Here:
\[
X_i \in [X_{\min}, X_{\max}], \quad Y_i \in [Y_{\min}, Y_{\max}], \quad Z_i = Z_{\text{fixed}}
\]
where:
\begin{itemize}
    \item \( X_{\min}, X_{\max} \): Define the range of the \( X \)-coordinate.
    \item \( Y_{\min}, Y_{\max} \): Define the range of the \( Y \)-coordinate.
    \item \( Z_{\text{fixed}} \): Represents a constant height for all waypoints.
\end{itemize}

For the purpose of situation coverage, the spatial range of the mine is defined as:
\[
X \in [X_{\min}, X_{\max}], \quad Y \in [Y_{\min}, Y_{\max}]
\]

A test case \( \sigma \) is defined as a tuple representing the state of the environment:
\[
\sigma = (O, L, P)
\]
where:
\begin{itemize}
    \item \( O \in \{0, 1\} \): Obstacle presence (\( O = 1 \) indicates an obstacle is present, \( O = 0 \) indicates no obstacle).
    \item \( L \in \{\text{High}, \text{Medium}, \text{Low}\} \): Light level of the environment.
    \item \( P \in \{\text{Detected}, \text{Not Detected}\} \): Person detection status.
\end{itemize}

The obstacle placement function \( f_O(O) \) determines whether an obstacle is present:
\[
f_O(O) =
\begin{cases}
P_o, & \text{if } O = 1 \\
\emptyset, & \text{if } O = 0
\end{cases}
\]
where:
\begin{itemize}
    \item \( P_o \): The physical position of the obstacle, sampled from a uniform distribution:
    \[
    P_o = (x_o, y_o, z_o), \quad x_o \sim U(X_{\min}, X_{\max}), \quad y_o \sim U(Y_{\min}, Y_{\max}), \quad z_o = 0
    \]
    \item \( \emptyset \): Indicates the absence of an obstacle.
\end{itemize}

The safety of the drone is evaluated using a collision detection function \( C(t) \), which determines whether a collision occurs at time \( t \). The safety condition over the entire journey \( T \) is defined as:
\[
S(\tau) = 1 - \max_{t \in [0, T]} C(t)
\]
where:
\begin{itemize}
    \item \( S(\tau) = 1 \): Indicates a safe journey with no collisions.
    \item \( S(\tau) = 0 \): Indicates a safety violation occurred during the journey.
\end{itemize}

The total number of test cases \( N_{\text{total}} \) is calculated as:
\[
N_{\text{total}} = |\Sigma| \times N_{\text{positions}}
\]
where:
\begin{itemize}
    \item \( |\Sigma| = |O| \times |L| \times |P| \): Total number of possible situations.
    \item \( N_{\text{positions}} \): Number of unique positions the drone visits.
\end{itemize}

The coverage percentage \( \kappa \) measures the ratio of total generated test cases in a run to the total number of possible test cases:
\[
\kappa = \frac{N_{\text{generated}}}{N_{\text{total}}} \times 100
\]
where:
\begin{itemize}
    \item \( N_{\text{generated}} \): Number of test cases where \( S(\tau) = 1 \).
    \item \( N_{\text{total}} \): Total number of possible test cases.
\end{itemize}




\begin{table}[h]
\centering
    
\begin{tabular}{p{4cm}p{4cm}p{4cm}}
    \includegraphics[width=0.34\textwidth,height=4cm]{Figure with no sitcov.png} &
        
    \includegraphics[width=0.32\textwidth,height=3.7cm]{Figure_with situation.png} &
        
    \includegraphics[width=0.33\textwidth,height=3.8cm]{Figure_with no light.png} \\
        
    (a) In normal condition & (b) With obstacles in default light  & (c) With obstacles in no light
        \\
\end{tabular}
    
\caption{Comparison of AAD's journey and behaviour in three different conditions.}\label{fig4}
    
\end{table}





\begin{framed}
\small
\begin{lstlisting}
1:  send("start_mission")  
2:  while not reached("final_waypoint") do  
3:      move_to("next_waypoint")  
4:      log("current_position")  
5:      generate("situation")  
6:      check("safety_violation")  
7:      log("original_result")  

8:      # Apply mutations  
        # Shift waypoint positions 
9:      mutate("waypoints")       
        # Change obstacle locations   
10:     mutate("obstacles")       
         # Modify sensor accuracy
11:     mutate("environment")  
         # Adjust detection thresholds 
12:     mutate("safety_params")   
13:     check("safety_violation_after_mutation")  
14: end while  
15: send("end_mission") 
\end{lstlisting}
\end{framed} 





In this study, we assessed the effectiveness of the SCALOFT testing approach using mutation testing to assess these variations, with the mutation score providing a reliable measure of a test set's ability to detect faults. Studies show that attaining a higher mutation score significantly enhances fault detection \cite{dos2024aat4irs,jia2010analysis,papadakis2018mutation}.

The system follows a linear sequence of commands that direct the AAD to move between waypoints while logging its position, detecting environmental situations, and verifying safety constraints. The program introduces controlled mutations at specific points, altering waypoints, obstacle locations, sensor accuracy, and safety parameters. These modifications assess the system’s robustness by comparing the original and mutated execution results. Since the code primarily consists of sequential commands for movement, logging, and safety checks, the injection points for mutations are limited.

We intend to conduct full-scale mutation testing of SCALOFT in simulation. However, as a first step, we performed unit testing with MutPy\footnote{https://github.com/mutpy/mutpy}, which generated 44 mutants. We evaluated their elimination using the control script's functions. The initial results show that out of a total of 44 mutants, SCALOFT successfully eliminated 30. This means SCALOFT successfully killed $68\%$ of the generated mutants, indicating its capability to detect critical faults (see Table \ref{tab:mutation_results}).However, a $68\%$ mutation score suggests that there is room for improvement in the test suite's effectiveness. To gain a more comprehensive understanding of its strength, we plan to introduce a larger and more diverse set of mutants in future iterations. By running multiple rounds of mutation testing and calculating the average mutation score, we aim to better assess and enhance SCALOFT’s fault detection capabilities. 

In this study, various operator modifications were introduced as mutations, potentially affecting the drone's navigation and safety mechanisms. The types of mutant used are- 

\begin{itemize}
    \item {Arithmetic Operator Deletion (AOD)} removes arithmetic operators (e.g., \texttt{+}, \texttt{-}, \texttt{*}, \texttt{/}).
    
    \item {Arithmetic Operator Replacement (AOR)} substitutes one arithmetic operator with another.
    
    \item {Conditional Operator Deletion (COD)} removes conditional statements (e.g., \texttt{if}, \texttt{else}).
    
    \item {Conditional Operator Insertion (COI)} introduces additional conditional checks, which may result in unnecessary constraints or altered decision flows, affecting system responsiveness.
    
    \item {Break Continue Replacement (BCR)} modifies \texttt{break} or \texttt{continue} statements, potentially disrupting loops that control iterative processes.
    
    \item{Assignment Operator Replacement (ASR)} changes assignment operators (e.g., \texttt{=}, \texttt{+=}, \texttt{-=}).
\end{itemize}

%The mutations covered different types of operator modifications that could impact the drone's navigation and safety mechanisms. Arithmetic Operator Deletion (AOD) and Arithmetic Operator Replacement (AOR) affected fundamental calculations, such as distance estimation and step counting, which are crucial for accurate motion planning. SCALOFT effectively detected and killed most of these mutants, ensuring the system's numerical computations remained robust. Conditional Operator Deletion (COD) and Conditional Operator Insertion (COI) introduced changes in decision-making logic, potentially leading to unsafe conditions, such as failing to recognize an obstacle. 
%However, some mutants survived, particularly those involving Break Continue Replacement (BCR) and Assignment Operator Replacement (ASR), suggesting potential gaps in testing related to lower-level operations or data handling. These results highlight SCALOFT's strengths in detecting critical numerical and decision-based faults while also indicating areas for further improvement, particularly in refining test cases to handle complex operator mutations.

\begin{table}[h!]
    \caption{Mutation Testing Results}
    \label{tab:mutation_results}
    \centering
    \begin{tabular}{|p{1.5cm}| p{4cm}| p{4cm}| c| c|}
        \hline
        \textbf{Mutant Type}  & \textbf{Modification}  & \textbf{Effect} & \textbf{Killed} & \textbf{Survived} \\
        \hline
        AOD  & Removes arithmetic operations (e.g., \texttt{distance = speed * time} $\rightarrow$ \texttt{distance = speed})  
             & Incorrect movement calculations, leading to wrong navigation paths or stuck behavior & 3  & 0  \\

        \hline
        AOR  & Replaces arithmetic operations (e.g., \texttt{+} $\rightarrow$ \texttt{-}, \texttt{*} $\rightarrow$ \texttt{/})  
             & Miscalculates distance and velocity,  causing erratic movements and inefficient path planning & 18 & 8 \\
        \hline
        ASR  & Changes how values are stored (e.g., \texttt{speed += 1} $\rightarrow$ \texttt{speed -= 1})  
             & The drone may slow down when it should speed up or misinterpret sensor updates, leading to delayed responses or unstable flight behavior & 1  & 1  \\
        \hline
        BCR  &   Impact loops (e.g. \texttt{break} $\rightarrow$ \texttt{continue}) 
             & Causes the drone to skip critical safety checks instead of aborting an unsafe mission & 0  & 2  \\
        \hline
        COD  & Removes conditions (e.g., \texttt{if (obstacle\_detected) stop();} $\rightarrow$ \texttt{stop();})  
             & Disables safety checks, making the drone ignore obstacles, leading to possible collisions or crashes & 4  & 0  \\
        \hline     
        COI  & Introduces unnecessary conditions (e.g., \texttt{if (battery > 50\%) land();})  
             & Creates unintended constraints, such as forcing the drone to land prematurely or refusing to move in certain conditions & 4  & 3  \\
        \hline
    \end{tabular}
\end{table}
 As autonomous systems operate in real-world environments, we introduced mutants to model possible variations in system behavior, especially in critical computational and decision-making processes. Mutants are small modifications made to a program’s source code or bytecode. If these changes go undetected by the test suite, it signals potential weaknesses in the testing process \cite{Andrews2005Mutation}. These alterations, known as mutations, are applied using predefined mutation operators that  mimic common programming errors (such as incorrect operators or variable names)
From Table \ref{tab:mutation_results}, we can see that SCALOFT effectively detected and eliminated most AOD, AOR, COD, and COI mutants, ensuring the system's numerical computations and decision-making logic remained robust. However, some mutants survived, particularly those involving BCR and ASR, indicating potential gaps in testing related to lower-level operations or data handling. To enhance SCALOFT’s test suite, we plan to refine test cases to specifically address these weaker areas by incorporating more comprehensive loop and data flow tests to detect issues caused by BCR mutations. Additionally, we will implement stronger assertions on variable updates and state transitions to catch ASR-related faults. Furthermore, we aim to introduce a broader range of mutation operators in future testing rounds to strengthen both numerical and logical components. By continuously expanding the mutation set and assessing test effectiveness, we seek to further improve SCALOFT’s fault detection capabilities and overall reliability in real-world deployment.



\begin{figure}[h!]
    \centering
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.25\textheight]{fault 1.JPG}
        
    \end{minipage}%
    \hfill
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.25\textheight]{fault 2.JPG}
        
    \end{minipage}%
    \hfill
    \begin{minipage}{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth, height=0.25\textheight]{fault 3.JPG}
        
    \end{minipage}
    \caption{Expected vs. Observed outcomes with three different seeded faults, each shown for three separate runs}
    \label{fig:faults}
\end{figure}



\begin{table}[h!]
    \centering
    \fontsize{8pt}{8pt}\selectfont
    \renewcommand{\arraystretch}{2} % Increase row spacing
    \caption{Expected vs. observed behavior after fault injections}
    \begin{tabular}{p{0.5cm}p{2.9cm}p{3.5cm}p{3.9cm}}
        \hline
       \textbf{ID}  & \textbf{Scenario} & \textbf{Expected Outcome} & \textbf{Observed Outcome}  \\
        \hline
        1  & 
        Delay the detection of a person by 3 seconds & 
        The drone reduces its speed 3 seconds late after detecting the person & 
      After detecting a person, the drone slows down for more than 3 seconds
          \\
         
       2  & 
        Every 20 seconds, simulate a false collision & 
         The drone will stop flying or get stuck, exhibiting a low-severity impact (scale 1)  &  
        The drone crashed and aborted the mission unexpectedly , indicating a high-severity impact (scale 3)
         \\
         
       3  & 
        Increase goal threshold (from default (0.15) to  0.5) & 
        The drone may stop before reaching waypoints leading to incorrect navigation & 
        The incorrect navigation led the drone to  collision 
          \\
      \hline   
    \end{tabular}
    \label{tab:fault_analysis}
\end{table} 


\begin{table}[ht]
\centering
\caption{Faults type considering HAZOP guidewords}
\begin{tabular}{p{0.5cm}p{4.5cm}p{6.5cm}}
\hline
\textbf{ID} &\textbf{Fault Type} & \textbf{HAZOP Guideword} \\
\hline
1 &Delayed Human Detection & LATE: Relative to the clock time  \\
2 &False Collision Signal & UNINTENDED: Unintended activation  \\
3 &Incorrect Goal Check Threshold & MORE: Quantitative increase\\
\hline
\end{tabular}
\label{tab:systematic fault}
\end{table}

